Stable-SCore: A Stable Registration-based Framework for 3D Shape Correspondence

Establishing character shape correspondence is a critical and fundamental task in computer vision and graphics, with diverse applications including re-topology, attribute transfer, and shape interpolation. Current dominant functional map methods, while effective in controlled scenarios, struggle in real situations with more complex challenges such as non-isometric shape discrepancies. In response, we revisit registration-for-correspondence methods and tap their potential for more stable shape correspondence estimation. To overcome their common issues including unstable deformations and the necessity for careful pre-alignment or high-quality initial 3D correspondences, we introduce Stable-SCore: A Stable Registration-based Framework for 3D Shape Correspondence. We first re-purpose a foundation model for 2D character correspondence that ensures reliable and stable 2D mappings. Crucially, we propose a novel Semantic Flow Guided Registration approach that leverages 2D correspondence to guide mesh deformations. Our framework significantly surpasses existing methods in challenging scenarios, and brings possibilities for a wide array of real applications, as demonstrated in our results.

==> tables/tab_ablation_2.tex <==
\begin{table}[h!]
    \centering
    \caption{Ablation study of different types of supervision given during registration.}
    \resizebox{0.50\textwidth}{!}{
    \begin{tabular}{lcc}
        \toprule
        \textbf{Method} & \textbf{Correpsondence PCK@0.1} & \textbf{Correpsondence PCK@0.02} \\
        \midrule
        SD+DINO                & 77.060  & 23.360  \\
        Telling left from right  & 68.050  & 21.610  \\
        Ours            & \textbf{95.230}  & \textbf{57.520}  \\
        \bottomrule
    \end{tabular}}
\end{table}
